Face Super-Resolution Using Stochastic Differential Equations

Diffusion models have proven effective for various applications such as images, audio and graph generation. Other important applications are image super-resolution and the solution of inverse problems. More recently, some works have used stochastic differential equations (SDEs) to generalize diffusion models to continuous time. In this work, we introduce SDEs to generate super-resolution face images. To the best of our knowledge, this is the first time SDEs have been used for such an application. The proposed method provides an improved peak signal-to-noise ratio (PSNR), structural similarity index measure (SSIM), and consistency than the existing super-resolution methods based on diffusion models. In particular, we also assess the potential application of this method for the face recognition task. A generic facial feature extractor is used to compare the super-resolution images with the ground truth and superior results were obtained compared with other methods. Our code is publicly available at https://github.com/marcelowds/sr-sde

==> 3-experiments.tex <==
\section{Experiments}
\label{sec:Experiments}
\HP{Eu juntaria as seções Experiments e Results  em "Experiments and Results". Se for esse o caso, devemos alterar a descrição no ultimo paragrafo da Introdução}
\DM{concordo. MS ou RL, please, do it!}

In this section, we describe the experiments performed to evaluate our method.
\cref{subseca} describes the methods and metrics used to verify the quality of the super-resolution images. 
\cref{subsecb} describes the experiments to verify the influence of different super-resolution methods on the face recognition task.
\cref{subsecc} describes the experimental parameters used in our experiments.

\subsection{Super-resolution}
\label{subseca}

To evaluate the capacity of \glspl*{sde} for the super-resolution task,  the four algorithms \gls*{sde}-\gls*{vp}, \gls*{sde}-subVP, \gls*{sde}-\gls*{ve} and \gls*{sde}-\gls*{ve}cs  are provided with $16\times 16$ images and produce  $128\times 128$ images. The working size of the network is $128 \times 128$, so the input is upsampled to this size. During training, low-quality images are obtained by downsampling the original high-resolution images by a factor of 8 and upsampling back to the original size.


To quantitatively evaluate the quality of the super-resolution images, the metrics \gls*{psnr} and \gls*{ssim} are used. We also use the consistency, defined as the \gls*{mse} between the down-sampled \gls*{sr} images and the low-resolution inputs.
Aiming to evaluate the potential applications of our method  on face recognition systems, we rely on the cosine similarity between the image features obtained from VGG-Face~\cite{vggface}.

Specifically for the \gls*{sde}-\gls*{ve}cs method, the Langevin correction depends on a parameter $r$ which controls the signal-to-noise ratio during the correction step.
Higher values of $r$ typically result in smoother images, as can be seen in \cref{fig_sr2}.
It is well known that the \gls*{psnr} and \gls*{ssim} metrics are not adequate for measuring the quality of super-resolution images because these metrics tend to be very conservative with high-frequency details~\cite{saharia2021image}.
Therefore, we use the \gls*{sde}-\gls*{ve}cs algorithm to generate a set of images with different values of $r$ and analyze the influence of the smoothness level on the \gls*{psnr} metric.
\begin{figure}[!ht]
\centering
\setlength{\tabcolsep}{2pt}

\begin{tabular}{cccc}
Original & Sample1 & Sample2 & Sample3 \\
\includegraphics[width=18mm]{figs/10-hr.png} & \includegraphics[width=18mm]{figs/10-sr_0.10.png} & \includegraphics[width=18mm]{figs/10-sr_0.30.png} & \includegraphics[width=18mm]{figs/10-sr_0.52.png} \\
\includegraphics[width=18mm]{figs/6-hr.png} & \includegraphics[width=18mm]{figs/6-sr_0.12.png} & \includegraphics[width=18mm]{figs/6-sr_0.32.png} & \includegraphics[width=18mm]{figs/6-sr_0.39.png}
\end{tabular}

\vspace{-1mm}

\caption{Samples obtained increasing $r$ from left to right. For Sample1, Sample2 and Sample3 the values of $r$ are $0.10$, $0.30$ and $0.52$ for the first row and $0.12$, $0.32$ and $0.39$ for the second row. Higher values of $r$ yield smoother images and larger values of \gls*{psnr} (on~average).}
\label{fig_sr2}
\end{figure}
\subsection{Feature extraction for face recognition}
\label{subsecb}

One application of super-resolution algorithms is face recognition.
In real-world scenarios, the images of surveillance cameras are usually noisy and low resolution~\cite{juefei2019, haghighat2017low, li2019low}.
Hence, considering that our method is based on denoising, we believe it can be very suitable for such~scenarios.

To evaluate the potential influence of the smoothness and \gls*{psnr} metric on the recognition accuracy, we also use different images obtained with the \gls*{sde}-\gls*{ve}cs algorithm for different values of $r$, analyzing which of these images are better for the face recognition task.
To compare the \gls*{sr} and \gls*{hr} images, we extract the features of the images using VGG-Face and measure the cosine similarity between~them. 

\JN{Not sure if this paragraph matters for the paper. Considering the target readers, everybody knows this.}
\DM{ok, but if we have room I guess it is good to be here}
Let $\mathbf{x}$ and $\tilde{\mathbf{x}}$ be the super-resolved and the original images, respectively. 
The features extracted with VGG-Face is a one-dimensional vector of size $F$ and can be denoted by $\mathbf{y}=f(\mathbf{x})$ for the super-resolution images and $\tilde{\mathbf{y}}=f(\tilde{\mathbf{x}})$ for the original images; $f(\cdot)$ is a feature extractor function. 
The cosine similarity between these two vectors is computed using
\begin{equation}
    s(\tilde{\mathbf{y}},\mathbf{y})=\frac{\langle \tilde{\mathbf{y}}, \mathbf{y}\rangle}{\|\tilde{\mathbf{y}}\|\cdot \|\mathbf{y}\|},
\end{equation}
where $\langle\cdot,\cdot\rangle$ denotes the scalar product, and $\|\cdot \|$ refers to the Euclidean norm. 
As the above similarity is calculated for $L$ images, we denote each feature vector by an index $i$. 
The average cosine similarity for the $L$ images, denoted by CS, is 
\begin{equation}
    \text{CS}=\frac{1}{L}\displaystyle\sum_{i=1}^Ls(\tilde{\mathbf{y}}_i,\mathbf{y}_i).
\end{equation}

CS is the result of facial feature extraction, so it strongly influences recognition accuracy.
CS values close to 1 indicate that the features of \gls*{sr} and \gls*{hr} images are very close and that the super-resolution algorithm is retrieving image details important for facial recognition.
Now one may ask what are the best super-resolution images to use on the recognition tasks, for example, the images with high-frequency details (smaller $r$) or smoother images (higher values of $r$).
To answer this question, we will analyze the influence of the $r$ parameter on the CS metric.
In this way, we can also analyze if there is relation between the values of CS and \gls*{psnr}. 


\subsection{Parameters and network training}
\label{subsecc}

Following~\cite{song2021score}, we set the parameters of the models as $\sigma_{min}=0.01$, $\sigma_{max}=348$, $\bar{\beta}_{min}=0.1$, and $\bar{\beta}_{min}=20.0$.
For the optimization, we used the Adam optimizer with a warm-up of $5000$ steps and a learning rate of~$2\times10^{-4}$.

For training, we explored the images from the \ffhq dataset~\cite{karras2019style} with $10^6$ steps. 
Due to the high execution time, for testing, we use a random sampling of $L=1024$ images of the CelebA-HQ dataset~\cite{karras2018progressive}. 
The total number of time steps is $N=2000$, and for the \gls*{sde}-\gls*{ve}cs, we used $M=2$ correction steps. 
For the VGG-Face feature extraction, a feature vector size of $F=512$ is~used.

All experiments were carried out on a computer with an AMD Ryzen $9$ $5950$X CPU ($3.4$GHz), $128$~GB of RAM ($2633$ MHz), and an NVIDIA GeForce RTX $3060$ GPU~($12$~GB).


==> 4-results.tex <==
\section{Results}
\label{sec:Results}

In this section, we analyze the influence of the parameter $r$ (related to the image smoothness) on the \gls*{psnr} and CS metrics.
We show that the peak in the \gls*{psnr} values does not coincide with the peak in the CS values; in other words, higher values of \gls*{psnr} do not imply higher values of CS.
We also demonstrate the superior quality of our method both qualitatively (with very detailed super-resolution images) and quantitatively (with the highest value for the CS metric), which is very important for recognition tasks.


Fig.~\ref{fig_psnr} shows \gls*{psnr} and CS as a function of the parameter~$r$.
As can be seen, higher values of $r$ cause the \gls*{psnr} to increase, with the highest value of \gls*{psnr} occurring at $r~\approx~0.5$.
Thus, with smoother images, we can obtain higher values of \gls*{psnr}.
This is in line with the regression model of~\cite{saharia2021image}, which provides blurry and less detailed images than SR3, but with better results for \gls*{psnr} and \gls*{ssim}. 

\JN{The use of question in the middle of the paragraph is not very common. This part should be restructured}
\DM{I agreed. MS, please fix it!}
As described in~\cite{johnson2016perceptual,zhang2018unreasonable}, the \gls*{psnr} metric does not align well with human perception. 
Nevertheless, for the recognition task, what is better: very detailed images with smaller \gls*{psnr} or smoother images  with higher \gls*{psnr}? 
To answer this question, we analyze CS, as a function of~$r$ in Fig.~\ref{fig_psnr}.
We observe that CS has a maximum value for $r~\approx~0.16$ (which is different from~$r$ for which \gls*{psnr} is maximum) and slightly decreases with~$r$.
We also computed the correlation coefficient between CS and \gls*{psnr} and obtained a value of $-0.6591$. 
Therefore, not always higher values of \gls*{psnr} are related to higher values of CS (and consequently higher recognition accuracy), as can be observed in the cross-plot between CS and \gls*{psnr} in \cref{fig_cs_psnr}.

\begin{figure}[!htb]
\centering
\includegraphics[width=0.9\linewidth]{figs/psnr_cs_vs_snr.pdf}

\vspace{-4mm}

\caption{CS and \gls*{psnr} as a function of $r$ (sampling parameter).
Higher values of $r$ produce smoother images (with higher values of \gls*{psnr}) but can decrease the value of~CS.}
\label{fig_psnr}
\end{figure}




\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\linewidth]{figs/cs_vs_psnr.pdf}

\vspace{-4mm}

\caption{Cross-plot between CS and \gls*{psnr}. The correlation coefficient between CS and \gls*{psnr}  is  $-0.6591$, implying that higher values of \gls*{psnr} do not always result in higher values of~CS.}
\label{fig_cs_psnr}
\end{figure}





\begin{table*}[!ht]
\caption{\gls*{psnr}, \gls*{ssim}, Consistency and CS on $16\times16 \rightarrow 128\times128$ face super-resolution. The best result for CS is highlighted with \red{red}.}
\label{metrics_table}
\centering

\vspace{-2mm}

\begin{tabular}{l c c c c}
\toprule
\textbf{Model} & \textbf{\gls*{psnr}} $\uparrow$ & \textbf{\gls*{ssim}} $\uparrow$ & \textbf{CONSISTENCY} $\downarrow$ & \textbf{CS} $\uparrow$\\
\midrule
\gfpgan~\cite{wang2021gfpgan} & $21.5326\pm 1.5273$ & $0.6006\pm 0.0709$ & $37.2256\pm 12.4622$ & $0.8689\pm 0.0581$\\
\sparnet~\cite{chen2020learning} & $24.3686\pm 1.7844$ & $0.7223\pm 0.0679$ & {$13.6512\pm \phantom{0}4.9063$} & $0.9307\pm 0.0301$\\
SR3~\cite{saharia2021image} & $22.9581\pm1.8370$ & $0.6605\pm0.0758$ & $\phantom{0}1.3715\pm \phantom{0}0.7904$& $0.9370\pm 0.0244$\\
\gls*{sde}-\gls*{vp} & $22.7171\pm1.8107$ & $0.6448\pm 0.0787$ & $\phantom{0}0.1074\pm \phantom{0}0.0592$ & $0.9330\pm 0.0262$\\
\gls*{sde}-subVP & $22.6455\pm 1.8047$ & $0.6428\pm 0.0797$ & $\phantom{0}0.1433\pm \phantom{0}0.1212$ & $0.9300\pm0.0261$\\
\gls*{sde}-\gls*{ve} & $23.5101\pm 1.9492$ & $0.6879\pm0.0797$ & $\phantom{0}0.0454\pm \phantom{0}0.0357$&\color{red}{$0.9443\pm 0.0222$}\\
\bottomrule
\end{tabular}
\end{table*}




\begin{figure*}[!htb]
\centering
\setlength{\tabcolsep}{2pt}

\resizebox{0.95\linewidth}{!}{ %
\begin{tabular}{ccccccccc}
Original & Input & \small{ \gfpgan~\cite{wang2021gfpgan}\phantom{i}} & \small{\sparnet~\cite{chen2020learning}} & SR3~\cite{saharia2021image} & \textcolor{blue}{SDE-VP} & \textcolor{blue}{SDE-subVP} & \textcolor{red}{SDE-VE} & \textcolor{blue}{SDE-VEcs} \\
\includegraphics[width=22mm]{figs/10-hr.png} & \includegraphics[width=22mm]{figs/10-lr.png} & \includegraphics[width=22mm]{figs/10-sr_gfpgan.png} & \includegraphics[width=22mm]{figs/10-sr_sparnet.png} & \includegraphics[width=22mm]{figs/10-sr_sr3.png} & \includegraphics[width=22mm]{figs/10-sr_vp_1M.png} & \includegraphics[width=22mm]{figs/10-sr_sub.png} & \includegraphics[width=22mm]{figs/10-sr_ve_1M.png} & \includegraphics[width=22mm]{figs/10-sr_ve_4c.png} \\
\includegraphics[width=22mm]{figs/36-hr.png} & \includegraphics[width=22mm]{figs/36-lr.png} & \includegraphics[width=22mm]{figs/36-sr_gfpgan.png} & \includegraphics[width=22mm]{figs/36-sr_sparnet.png} &  \includegraphics[width=22mm]{figs/36-sr_sr3.png} & \includegraphics[width=22mm]{figs/36-sr_vp_1M.png} & \includegraphics[width=22mm]{figs/36-sr_sub.png} & \includegraphics[width=22mm]{figs/36-sr_ve_1M.png} & \includegraphics[width=22mm]{figs/36-sr_ve_4c.png} \\
\includegraphics[width=22mm]{figs/6-hr.png} & \includegraphics[width=22mm]{figs/6-lr.png} & \includegraphics[width=22mm]{figs/6-sr_gfpgan.png} & \includegraphics[width=22mm]{figs/6-sr_sparnet.png} & \includegraphics[width=22mm]{figs/6-sr_sr3.png} & \includegraphics[width=22mm]{figs/6-sr_vp_1M.png} & \includegraphics[width=22mm]{figs/6-sr_sub.png} & \includegraphics[width=22mm]{figs/6-sr_ve_1M.png} & \includegraphics[width=22mm]{figs/6-sr_ve_4c.png} \\
\includegraphics[width=22mm]{figs/81-hr.png} & \includegraphics[width=22mm]{figs/81-lr.png} & \includegraphics[width=22mm]{figs/81-sr_gfpgan.png} & \includegraphics[width=22mm]{figs/81-sr_sparnet.png} & \includegraphics[width=22mm]{figs/81-sr_sr3.png} & \includegraphics[width=22mm]{figs/81-sr_vp_1M.png} & \includegraphics[width=22mm]{figs/81-sr_sub.png} & \includegraphics[width=22mm]{figs/81-sr_ve_1M.png} & \includegraphics[width=22mm]{figs/81-sr_ve_4c.png} \\
\includegraphics[width=22mm]{figs/536-hr.png} & \includegraphics[width=22mm]{figs/536-lr.png} & \includegraphics[width=22mm]{figs/536-sr_gfpgan.png} & \includegraphics[width=22mm]{figs/536-sr_sparnet.png} & \includegraphics[width=22mm]{figs/536-sr_sr3.png} & \includegraphics[width=22mm]{figs/536-sr_vp_1M.png} & \includegraphics[width=22mm]{figs/536-sr_sub.png} & \includegraphics[width=22mm]{figs/536-sr_ve_1M.png} & \includegraphics[width=22mm]{figs/536-sr_ve_4c.png} \\
\includegraphics[width=22mm]{figs/930-hr.png} & \includegraphics[width=22mm]{figs/930-lr.png} & \includegraphics[width=22mm]{figs/930-sr_gfpgan.png} & \includegraphics[width=22mm]{figs/930-sr_sparnet.png} & \includegraphics[width=22mm]{figs/930-sr_sr3.png} & \includegraphics[width=22mm]{figs/930-sr_vp_1M.png} & \includegraphics[width=22mm]{figs/930-sr_sub.png} & \includegraphics[width=22mm]{figs/930-sr_ve_1M.png} & \includegraphics[width=22mm]{figs/930-sr_ve_4c.png}
\end{tabular}
}

\vspace{-1mm}

\caption{Super-resolution results. Our methods are shown in \red{red} (the best) and \blue{blue}. \red{SDE-VE} provides more natural and detailed images than other methods. It is worth highlighting that \blue{\gls*{sde}-\gls*{ve}cs} can even retrieve finer details in some cases, such as the beard in the image shown in the fifth row.}
\label{fig_sr}
\end{figure*}


We also evaluate the proposed methods qualitatively (visually) in \cref{fig_sr}, where it is demonstrated that the recovered images with SDE-VE have, in most cases, more quality, more high-frequency details, and are more natural when compared with other methods.
The \sparnet method~\cite{chen2020learning} generates images without distortion, but smoother when compared with  our four methods. For some images, our SDE-VEcs method is able recover even the finest details, such as the beard in the image shown in the fifth row of~\cref{fig_sr}. 

To evaluate our results quantitatively, we present in Table~\ref{metrics_table} the metrics \gls*{psnr}, \gls*{ssim}, consistency and CS.
The \sparnet method~\cite{chen2020learning} achieves the highest value of \gls*{psnr} and \gls*{ssim}, but as discussed earlier, this is not enough to generate images with high-frequency details as it occurs in SR3~\cite{saharia2021image} and in the variations of the proposed approach.
As we are interested in applying our super-resolution method for surveillance scenarios and facial recognition, we are interested in recovering details that maximize the CS metric.
As we can see in Table \ref{metrics_table}, the method SDE-VE achieves the highest value for the CS metric, supporting the idea that the SDE-VE method has better performance than other super-resolution methods for the face recognition task.
When comparing our four methods based on \glspl*{sde} presented here, the SDE-VE has the best results. 














